When Can Test-Time Adaptation Help Zero-Shot CT Vision-Language Models?

3D CT vision-language models (VLMs) classify abnormalities from text prompts in a zero-shot manner, enabling cross-institution deployment where labels are scarce and clinical tasks shift faster than supervised models can be retrained. A real CT scan, however, typically contains several co-occurring abnormalities, and the reliability of zero-shot multi-label prediction under distribution shift remains poorly understood. Test-time adaptation (TTA) updates a model on unlabeled target scans without source data or target annotations, yet existing TTA methods target multi-class softmax prediction on natural images or 2D medical segmentation, and none addresses unsupervised multi-label adaptation for zero-shot 3D CT VLMs. We study when TTA helps zero-shot 3D CT VLMs. A controlled diagnostic analysis shows that TTA is conditional: the volumetric input must preserve the encoder's depth structure, and the base representation must transfer to the target cohort, with depth reduction alone lowering internal AUROC by more than 0.12. We then focus on the regime where the base model already separates present from absent abnormalities. We introduce CARVE (Cardinality-Aware Retained-View Entropy), the first TTA method for this setting. CARVE estimates a sample-specific positive-label cardinality $\hat{k}$, optimizes a top-$\hat{k}$ objective to preserve co-occurring abnormalities, and performs memory-efficient multi-view adaptation by scoring weak 3D views without gradients before updating on a retained subset. Across contrastive CT-CLIP and anatomy-aware fVLM, CARVE provides the most consistent improvements across multi-label, three-class, and binary CT tasks when the base model is already discriminative. These results establish multi-label TTA for zero-shot 3D CT VLMs as a distinct problem and CARVE as a cardinality-aware solution.

==> images/analysis.tex <==
\begin{figure}[t]
    \centering \includegraphics[width=\linewidth]{images/CARVE-intro.pdf}
    \caption{\textbf{TTA for zero-shot 3D CT VLMs is conditional.}
Adaptation helps only when the input preserves volumetric structure, the backbone transfers well, and the objective matches multi-label prediction. Preserving native input, using a stronger base model, and optimizing CARVE's cardinality-aware objective consistently improve AUROC.}
\label{fig:intro_diagnostic}
\end{figure}

==> sec/3_multilabel.tex <==
% % =====================================================================
% \section{Why Entropy Minimization Misfits Multi-Label 3D CT}
% \label{sec:multilabel}

% A test-time adaptation method inherits the assumptions of its objective.
% The objective that dominates the literature, prediction-entropy
% minimization, was designed for a setting that 3D CT abnormality
% detection does not satisfy. We make the mismatch precise, because it is
% the reason a cardinality-aware objective is needed rather than a
% convenience.

% \subsection{Prompt-pair scoring yields independent Bernoullis}
% A zero-shot 3D CT VLM scores each candidate finding through a pair of
% textual prompts. For label $j\!\in\!\{1,\dots,L\}$ we construct a
% positive prompt $t_j^{+}$ and a negative prompt $t_j^{-}$ asserting the
% presence and absence of the finding, read off image--text similarities
% $s_j^{+}(x;\theta)$ and $s_j^{-}(x;\theta)$, and convert their margin
% $d_j\!=\!s_j^{+}\!-\!s_j^{-}$ into a presence probability through a
% two-class softmax, equivalently a logistic:
% \begin{equation}
% p_j(x;\theta)=\frac{\exp(s_j^{+})}{\exp(s_j^{-})+\exp(s_j^{+})}=\sigma(d_j).
% \label{eq:ppair}
% \end{equation}
% The model thus emits a vector $\mathbf{p}=[p_1,\dots,p_L]\in[0,1]^L$ of
% \emph{independent} Bernoulli probabilities, one per finding. There is no
% normalization across labels: $\sum_j p_j$ is unconstrained and routinely
% exceeds one, because a single scan can present several co-occurring
% abnormalities. This is the defining structure of multi-label diagnosis,
% and it is exactly what a single categorical softmax cannot represent.

% \subsection{Tent assumes a structure that is absent}
% Tent~\cite{wang2021tent} and its descendants minimize the entropy of a
% softmax over mutually exclusive classes, $H(\mathbf{p})=-\sum_c p_c\log
% p_c$, updating only normalization parameters. Carrying this objective
% into prompt-pair scoring forces one of two assumptions, and both are
% wrong for CT.

% \paragraph{(i) A cross-label categorical.}
% Treating the $L$ positive logits as one categorical distribution and
% minimizing its entropy moves probability mass toward the single most
% confident finding and away from every other. This is the
% one-correct-class assumption made explicit: it actively \emph{suppresses}
% secondary positives, the co-occurring abnormalities a multi-label model
% exists to detect. The same winner-take-all pathology was identified for
% 2D natural images by ML-TTA~\cite{wu2025mltta}.

% \paragraph{(ii) Per-pair binary entropy.}
% Minimizing the binary entropy $h(p_j)=-p_j\log p_j-(1\!-\!p_j)\log(1\!-\!p_j)$
% of each Bernoulli independently avoids the collapse but inherits a
% different failure. Its gradient $\mathrm{d}h/\mathrm{d}p=\log\frac{1-p}{p}$
% vanishes at $p\!=\!0.5$ and only sharpens whichever side a label already
% leans toward. Under external shift, prompt-pair probabilities concentrate
% near $0.5$, precisely where this gradient is weakest, so the update is
% dominated by noise where it is not simply inert, and it carries no
% information about how many findings a scan should contain.

% \subsection{The missing quantity is cardinality}
% Both failures share a root cause: entropy objectives do not model the
% \emph{number} of positive labels per scan. A categorical entropy
% implicitly fixes that number at one; independent binary entropy treats
% every label as separately certain. Neither matches the empirical regime,
% where the positive count varies from one to roughly six co-occurring
% findings per scan. A correct test-time objective for multi-label 3D CT
% must therefore (i) preserve multiple likely positives instead of
% collapsing toward a single dominant label, and (ii) estimate a
% sample-specific cardinality $\hat{k}$ to decide how many to preserve.
% CARVE (Section~\ref{sec:method}) is built around exactly these two
% requirements, recovering Tent and ML-TTA as limiting cases when the
% estimated cardinality is degenerate.

